Understanding Cross-Domain Few-Shot Learning Based on Domain Similarity and Few-Shot Difficulty

Cross-domain few-shot learning (CD-FSL) has drawn increasing attention for handling large differences between the source and target domains--an important concern in real-world scenarios. To overcome these large differences, recent works have considered exploiting small-scale unlabeled data from the target domain during the pre-training stage. This data enables self-supervised pre-training on the target domain, in addition to supervised pre-training on the source domain. In this paper, we empirically investigate which pre-training is preferred based on domain similarity and few-shot difficulty of the target domain. We discover that the performance gain of self-supervised pre-training over supervised pre-training becomes large when the target domain is dissimilar to the source domain, or the target domain itself has low few-shot difficulty. We further design two pre-training schemes, mixed-supervised and two-stage learning, that improve performance. In this light, we present six findings for CD-FSL, which are supported by extensive experiments and analyses on three source and eight target benchmark datasets with varying levels of domain similarity and few-shot difficulty. Our code is available at https://github.com/sungnyun/understanding-cdfsl.

==> table/difficulty.tex <==
\begin{table*}[t]
\caption{5way-$k$shot performance of the designed cases to quantify the data difficulty. (a) No pre-training \& classifier fine-tuning (i.e., random feature). (b) No pre-training \& entire network fine-tuning. ResNet10 is used as a backbone.}\label{tab:difficulty}
\vskip 0.10in
\centering
\footnotesize
\begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 26.93{\scriptsize$\pm$.62} & 47.00{\scriptsize$\pm$.91} & 30.52{\scriptsize$\pm$.66} & 41.77{\scriptsize$\pm$.65} & 22.31{\scriptsize$\pm$.32} & 27.29{\scriptsize$\pm$.48} & 20.36{\scriptsize$\pm$.24} & 21.28{\scriptsize$\pm$.30} \\
    (b) & 51.00{\scriptsize$\pm$.88} & 77.65{\scriptsize$\pm$.72} & 44.63{\scriptsize$\pm$.87} & 56.45{\scriptsize$\pm$.84} & 25.87{\scriptsize$\pm$.51} & 40.22{\scriptsize$\pm$.60} & 21.05{\scriptsize$\pm$.35} & 22.28{\scriptsize$\pm$.39} \\
    \midrule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{Plantae} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{Cars} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 25.13{\scriptsize$\pm$.47} & 35.25{\scriptsize$\pm$.57} & 24.17{\scriptsize$\pm$.42} & 32.83{\scriptsize$\pm$.54} & 23.98{\scriptsize$\pm$.45} & 31.28{\scriptsize$\pm$.56} & 21.83{\scriptsize$\pm$.34} & 26.58{\scriptsize$\pm$.48} \\
    (b) & 29.98{\scriptsize$\pm$.59} & 38.93{\scriptsize$\pm$.58} & 27.04{\scriptsize$\pm$.53} & 39.00{\scriptsize$\pm$.62} & 27.14{\scriptsize$\pm$.53} & 36.93{\scriptsize$\pm$.64} & 24.78{\scriptsize$\pm$.48} & 33.36{\scriptsize$\pm$.58} \\
    \bottomrule
\end{tabular}
\end{table*}

==> table/homo_tl_mtl.tex <==
\begin{table*}[h]
\caption{5way-$k$shot performance of the designed upper performance cases. (a) SL pre-training with 20\% of target data as labeled data, (b) SSL pre-training (SimCLR) with 20\% of target data as unlabeled data, and (c) MSL pre-training (SL+SimCLR) with 20\% of target data as both labeled and unlabeled data. We fixed $\gamma=0.5$ in MSL. ResNet10 is used as a backbone.}\label{tab:homo_tl_mtl}
\vskip 0.10in
\centering
\footnotesize
\begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 92.44{\scriptsize$\pm$.55} & 99.00{\scriptsize$\pm$.15} & 83.34{\scriptsize$\pm$.68} & 95.37{\scriptsize$\pm$.26} & 42.89{\scriptsize$\pm$.77} & 56.94{\scriptsize$\pm$.65} & \textbf{28.89}{\scriptsize$\pm$.55} & \textbf{36.59}{\scriptsize$\pm$.56} \\
    (b) & 89.49{\scriptsize$\pm$.74} & 97.24{\scriptsize$\pm$.33} & 79.50{\scriptsize$\pm$.78} & 92.36{\scriptsize$\pm$.37} & 34.90{\scriptsize$\pm$.64} & 46.76{\scriptsize$\pm$.61} & 21.97{\scriptsize$\pm$.41} & 25.62{\scriptsize$\pm$.43} \\
    (c) & \textbf{96.57}{\scriptsize$\pm$.38} & \textbf{99.47}{\scriptsize$\pm$.11} & \textbf{85.99}{\scriptsize$\pm$.64} & \textbf{96.07}{\scriptsize$\pm$.24} & \textbf{43.53}{\scriptsize$\pm$.77} & \textbf{57.62}{\scriptsize$\pm$.67} & 26.92{\scriptsize$\pm$.50} & 35.39{\scriptsize$\pm$.54} \\
    \midrule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{Plantae} & \multicolumn{2}{c}{Cars} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 57.25{\scriptsize$\pm$.82} & 77.39{\scriptsize$\pm$.63} & 40.72{\scriptsize$\pm$.73} & 60.29{\scriptsize$\pm$.78} & 49.08{\scriptsize$\pm$.83} & 70.56{\scriptsize$\pm$.76}  & 43.32{\scriptsize$\pm$.72} & 66.40{\scriptsize$\pm$.68} \\
    (b) & 58.75{\scriptsize$\pm$.93} & 78.39{\scriptsize$\pm$.61} & 35.49{\scriptsize$\pm$.73} & 47.69{\scriptsize$\pm$.77} & 42.65{\scriptsize$\pm$.80} & 59.77{\scriptsize$\pm$.82}  & 28.67{\scriptsize$\pm$.71} & 38.34{\scriptsize$\pm$.67} \\
    (c) & \textbf{62.49}{\scriptsize$\pm$.87} & \textbf{80.84}{\scriptsize$\pm$.57} & \textbf{41.31}{\scriptsize$\pm$.76} & \textbf{60.50}{\scriptsize$\pm$.79} & \textbf{52.76}{\scriptsize$\pm$.87} & \textbf{73.75}{\scriptsize$\pm$.73}  & \textbf{47.61}{\scriptsize$\pm$.81} & \textbf{71.06}{\scriptsize$\pm$.69} \\
    \bottomrule
\end{tabular}
\end{table*}

==> table/homo_tl_mtl_byol.tex <==
\begin{table}[h]
\caption{5way-$k$shot performance of the designed upper performance cases. (a) SL pre-training with 20\% of target data as labeled data, (b) SSL pre-training (BYOL) with 20\% of target data as unlabeled data, and (c) MSL pre-training (SL+BYOL) with 20\% of target data as both labeled and unlabeled data. ResNet10 is used as a backbone.}\label{tab:homo_tl_mtl_byol}
\vskip 0.10in
\centering
\footnotesize
\begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & \textbf{92.44}{\scriptsize$\pm$.55} & \textbf{99.00}{\scriptsize$\pm$.15} & \textbf{83.34}{\scriptsize$\pm$.68} & \textbf{95.37}{\scriptsize$\pm$.26} & \textbf{42.89}{\scriptsize$\pm$.77} & \textbf{56.94}{\scriptsize$\pm$.65} & \textbf{28.89}{\scriptsize$\pm$.55} & 36.59{\scriptsize$\pm$.56} \\
    (b) & 80.10{\scriptsize$\pm$.76} & 94.53{\scriptsize$\pm$.41} & 66.45{\scriptsize$\pm$.80} & 86.55{\scriptsize$\pm$.50} & 33.50{\scriptsize$\pm$.59} & 45.99{\scriptsize$\pm$.63} & 23.11{\scriptsize$\pm$.42} & 27.71{\scriptsize$\pm$.44} \\
    (c) & 89.80{\scriptsize$\pm$.60} & 97.77{\scriptsize$\pm$.24} & 79.34{\scriptsize$\pm$.71} & 93.59{\scriptsize$\pm$.34} & 41.44{\scriptsize$\pm$.74} & 55.62{\scriptsize$\pm$.66} & 28.65{\scriptsize$\pm$.55} & \textbf{36.78}{\scriptsize$\pm$.55} \\
    \midrule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{Plantae} & \multicolumn{2}{c}{Cars} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) &  57.25{\scriptsize$\pm$.82} & 77.39{\scriptsize$\pm$.63} &
    \textbf{40.72}{\scriptsize$\pm$.73} & \textbf{60.29}{\scriptsize$\pm$.78} &  \textbf{49.08}{\scriptsize$\pm$.83} & \textbf{70.56}{\scriptsize$\pm$.76}  & 
    \textbf{43.32}{\scriptsize$\pm$.72} & \textbf{66.40}{\scriptsize$\pm$.68} \\
    (b) & 47.81{\scriptsize$\pm$.75} & 68.14{\scriptsize$\pm$.68}&
    35.96{\scriptsize$\pm$.70}& 49.34{\scriptsize$\pm$.76}&  39.12{\scriptsize$\pm$.71}& 55.31{\scriptsize$\pm$.79} &
    27.68{\scriptsize$\pm$.62}& 37.33{\scriptsize$\pm$.59} \\
    (c) & \textbf{58.74}{\scriptsize$\pm$.85} & \textbf{78.04}{\scriptsize$\pm$.58}& 36.47{\scriptsize$\pm$.73}& 55.70{\scriptsize$\pm$.73}& 44.56{\scriptsize$\pm$.79}& 66.57{\scriptsize$\pm$.78}& 39.32{\scriptsize$\pm$.73}& 60.16{\scriptsize$\pm$.72} \\
    \bottomrule
\end{tabular}
\end{table}

==> table/main_two_stage_bscd.tex <==
\begin{table*}[t]
\caption{$5$way-$k$shot performance of baselines and recent CD-FSL algorithms (\autoref{sec:analysis3}). ResNet10 is used as a backbone. Mean and 95\% confidence interval over 600 episodes are reported.}\label{tab:twostage}
\vskip 0.10in
\centering
\footnotesize\addtolength{\tabcolsep}{-2pt}
\begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Method} & \multirow{2}{*}{$\gamma$} & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & & & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    \multirow{2}{*}{SSL} & SimCLR & - & 89.49{\scriptsize$\pm$.74} & 97.24{\scriptsize$\pm$.33} & 79.50{\scriptsize$\pm$.78} & 92.36{\scriptsize$\pm$.37} & 34.90{\scriptsize$\pm$.64} & 46.76{\scriptsize$\pm$.61} & 21.97{\scriptsize$\pm$.41} & 25.62{\scriptsize$\pm$.43} \\
    & BYOL & - & 80.10{\scriptsize$\pm$.76} & 94.53{\scriptsize$\pm$.41} & 66.45{\scriptsize$\pm$.80} & 86.55{\scriptsize$\pm$.50} & 33.50{\scriptsize$\pm$.59} & 45.99{\scriptsize$\pm$.63} & 23.11{\scriptsize$\pm$.42} & 27.71{\scriptsize$\pm$.44} \\
    \midrule
    \multirow{4}{*}{SL $\rightarrow$ SSL} & SimCLR & - & \textbf{89.39}{\scriptsize$\pm$.82} & \textbf{96.84}{\scriptsize$\pm$.40} & \textbf{82.64}{\scriptsize$\pm$.73} & \textbf{94.51}{\scriptsize$\pm$.32} & 35.09{\scriptsize$\pm$.64} & 48.23{\scriptsize$\pm$.59} & 22.15{\scriptsize$\pm$.40} & 24.59{\scriptsize$\pm$.42} \\
    & MoCo & - & 83.26{\scriptsize$\pm$.88} & 93.93{\scriptsize$\pm$.47} & 76.87{\scriptsize$\pm$.84} & 90.05{\scriptsize$\pm$.48} & 32.67{\scriptsize$\pm$.62} & 44.51{\scriptsize$\pm$.59} & 22.02{\scriptsize$\pm$.41} & 26.44{\scriptsize$\pm$.46} \\
    & BYOL & - & 82.61{\scriptsize$\pm$.76} & 95.87{\scriptsize$\pm$.35} & 67.67{\scriptsize$\pm$.77} & 90.01{\scriptsize$\pm$.43} & \textbf{35.92}{\scriptsize$\pm$.68} & \textbf{50.33}{\scriptsize$\pm$.67} & 23.76{\scriptsize$\pm$.45} & 29.94{\scriptsize$\pm$.48} \\
    & SimSiam & - & 83.38{\scriptsize$\pm$.78} & 95.94{\scriptsize$\pm$.35} & 68.14{\scriptsize$\pm$.79} & 90.56{\scriptsize$\pm$.42} & 34.87{\scriptsize$\pm$.63} & 50.00{\scriptsize$\pm$.65} & \textbf{24.22}{\scriptsize$\pm$.45} & \textbf{30.58}{\scriptsize$\pm$.51} \\
    \midrule
    \multirow{6}{*}{\shortstack{SL $\rightarrow$ MSL \\ (Baseline)}} & \multirow{3}{*}{SimCLR} & 1/4 & 79.31{\scriptsize$\pm$.84} & 93.81{\scriptsize$\pm$.43} & 70.05{\scriptsize$\pm$.84} & 87.70{\scriptsize$\pm$.51} & 33.63{\scriptsize$\pm$.63} & 46.71{\scriptsize$\pm$.62} & 22.63{\scriptsize$\pm$.42} & 27.14{\scriptsize$\pm$.42} \\
    & & 2/4 & 82.12{\scriptsize$\pm$.78} & 94.91{\scriptsize$\pm$.42} & 71.48{\scriptsize$\pm$.81} & 88.86{\scriptsize$\pm$.44} & 34.38{\scriptsize$\pm$.65} & 47.34{\scriptsize$\pm$.64} & 22.82{\scriptsize$\pm$.41} & 26.81{\scriptsize$\pm$.44} \\
    & & 3/4 & 84.74{\scriptsize$\pm$.80} & 96.19{\scriptsize$\pm$.36} & 75.97{\scriptsize$\pm$.79} & 91.11{\scriptsize$\pm$.39} & 34.79{\scriptsize$\pm$.66} & 47.99{\scriptsize$\pm$.60} & 22.85{\scriptsize$\pm$.43} & 26.85{\scriptsize$\pm$.44} \\
    & \multirow{3}{*}{BYOL} & 1/4 & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} \\
    & & 2/4 & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} & xx.xx{\scriptsize$\pm$.xx} \\
    & & 3/4 & 76.08{\scriptsize$\pm$.84} & 93.94{\scriptsize$\pm$.42} & 67.39{\scriptsize$\pm$.81} & 87.90{\scriptsize$\pm$.48} & 34.46{\scriptsize$\pm$.65} & 47.88{\scriptsize$\pm$.65} & 23.78{\scriptsize$\pm$.43} & 28.83{\scriptsize$\pm$.48} \\
    \midrule
    \multirow{3}{*}{SL $\rightarrow$ MSL} & CHEF \yrcite{adler2020cross} & - & - & 86.87{\scriptsize$\pm$.27} & - & 74.15{\scriptsize$\pm$.27} & - & 41.26{\scriptsize$\pm$.34} & - & 24.72{\scriptsize$\pm$.14} \\
    & STARTUP \yrcite{phoo2021selftraining} & - & 75.93{\scriptsize$\pm$.80} & 93.02{\scriptsize$\pm$.45} & 63.88{\scriptsize$\pm$.84} & 82.29{\scriptsize$\pm$.60} & 32.66{\scriptsize$\pm$.60} & 47.22{\scriptsize$\pm$.61} & 23.09{\scriptsize$\pm$.43} & 26.94{\scriptsize$\pm$.44} \\
    & DD \yrcite{islam2021dynamic} & - & 82.14{\scriptsize$\pm$.78} & 95.54{\scriptsize$\pm$.38} & 73.14{\scriptsize$\pm$.84} & 89.07{\scriptsize$\pm$.47} & 34.66{\scriptsize$\pm$.58} & 49.36{\scriptsize$\pm$.59} & 23.38{\scriptsize$\pm$.43} & 28.31{\scriptsize$\pm$.46} \\
    \bottomrule
\end{tabular}
\end{table*}

==> table/sl_similarity.tex <==
\begin{table*}[t]
\caption{5way-$k$shot performance of the designed upper performance cases. (a) SL pre-training with 20\% of target data as labeled data, (b) SSL pre-training (SimCLR) with 20\% of target data as unlabeled data, and (c) MSL pre-training (SL+SimCLR) with 20\% of target data as both labeled and unlabeled data. We fixed $\gamma=0.5$ in MSL. ResNet10 is used as a backbone.}\label{tab:homo_tl_mtl}
\vskip 0.10in
\centering
\footnotesize
\begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{CropDisease} & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 92.44{\scriptsize$\pm$.55} & 99.00{\scriptsize$\pm$.15} & 83.34{\scriptsize$\pm$.68} & 95.37{\scriptsize$\pm$.26} & 42.89{\scriptsize$\pm$.77} & 56.94{\scriptsize$\pm$.65} & \textbf{28.89}{\scriptsize$\pm$.55} & \textbf{36.59}{\scriptsize$\pm$.56} \\
    (b) & 89.49{\scriptsize$\pm$.74} & 97.24{\scriptsize$\pm$.33} & 79.50{\scriptsize$\pm$.78} & 92.36{\scriptsize$\pm$.37} & 34.90{\scriptsize$\pm$.64} & 46.76{\scriptsize$\pm$.61} & 21.97{\scriptsize$\pm$.41} & 25.62{\scriptsize$\pm$.43} \\
    (c) & \textbf{96.57}{\scriptsize$\pm$.38} & \textbf{99.47}{\scriptsize$\pm$.11} & \textbf{85.99}{\scriptsize$\pm$.64} & \textbf{96.07}{\scriptsize$\pm$.24} & \textbf{43.53}{\scriptsize$\pm$.77} & \textbf{57.62}{\scriptsize$\pm$.67} & 26.92{\scriptsize$\pm$.50} & 35.39{\scriptsize$\pm$.54} \\
    \midrule
    \multirow{2}{*}{Case} & \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{Plantae} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{Cars} \\
    & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 & $k$=1 & $k$=5 \\
    \midrule
    (a) & 57.25{\scriptsize$\pm$.82} & 77.39{\scriptsize$\pm$.63} & 49.08{\scriptsize$\pm$.83} & 70.56{\scriptsize$\pm$.76} & 40.72{\scriptsize$\pm$.73} & 60.29{\scriptsize$\pm$.78} & 43.32{\scriptsize$\pm$.72} & 66.40{\scriptsize$\pm$.68} \\
    (b) & 58.75{\scriptsize$\pm$.93} & 78.39{\scriptsize$\pm$.61} & 42.65{\scriptsize$\pm$.80} & 59.77{\scriptsize$\pm$.82} & 35.49{\scriptsize$\pm$.73} & 47.69{\scriptsize$\pm$.77} & 28.67{\scriptsize$\pm$.71} & 38.34{\scriptsize$\pm$.67} \\
    (c) & \textbf{62.49}{\scriptsize$\pm$.87} & \textbf{80.84}{\scriptsize$\pm$.57} & \textbf{52.76}{\scriptsize$\pm$.87} & \textbf{73.75}{\scriptsize$\pm$.73} & \textbf{41.31}{\scriptsize$\pm$.76} & \textbf{60.50}{\scriptsize$\pm$.79} & \textbf{47.61}{\scriptsize$\pm$.81} & \textbf{71.06}{\scriptsize$\pm$.69} \\
    \bottomrule
\end{tabular}
\end{table*}
